La R\'esistance: Harnessing Heterogeneous Resources for Adaptive Resiliency in 6G Networks

Recent years have seen more critical applications designed to protect human lives (e.g., environmental sensing, emergency response, and tactical defense) being deployed over wireless networks. These critical deployments expect higher data rates, ultra-low latency, and ultra-high reliability. 6G wireless networks are expected to fill the gap in terms of the first two aspects (i.e., higher data rates and ultra-low latency), however providing ultra-high reliability is a wide open challenge. All is well when everything works but when there is a failure or a security attack, the entire system collapses exposing the associated human lives to imminent danger. Avoiding this requires the strongest of assurances that safety and security aspects are protected no matter what. Large scale critical applications are waiting for this piece of the puzzle to be solved. At this juncture, we envision the bold theme of La R\'esistance 6G (LR6G) that would pave the way for deploying mission-critical applications and services over 6G networks. It aims to achieve ultra-high reliability and resiliency to any disruptions, be it failures or security attacks. A few disruptions are easy to handle such as a cloud VM or primary link failure. In both of these cases, applications can be restored by activating the standby resource. However, some disruptions can be detrimental such as when a cut-vertex fails or when the disruption leaves the critical application to fail without access to a standby resource. These critical applications (e.g. Smart Manufacturing, Smart City, Ocean monitoring, Wildfire monitoring, etc.) are highly distributed in nature. They must continue to deliver their mission objectives during a disruption to protect human lives. In this paper, we present our LR6G vision and outline the challenges towards achieving this vision.

==> sections/integ.tex <==
\subsection{Integration}
So far, the individual components of our 6G architecture and their challenges were presented. How these components work together to meet the overall objective is presented here. This section describes two phases. The first phase is the preparatory phase and the second one is the adaptation phase. 

The preparatory phase encompasses system level interactions before a disruption happens. In this phase, individual components discover and acquire the knowledge required to adapt to a disruptive event as shown in Fig.~\ref{fig:preparatory}.

\begin{figure*}[htb]
  \centering
  \includegraphics[trim=0 120 0 0,clip,width=\textwidth]{figs/rings-b4disruption.png}
  \vspace{5mm}
  \caption{Preparatory phase \raj{if we have space, make this bigger}}
  \vspace{1mm}
  \label{fig:preparatory}
\end{figure*}

ASSESS component requires a detailed capability and capacity discovery whenever there is a change in the full-stack. This does not change frequently. 
\joaquin{On wireless environments this will change very frequently, as the SNR of the channel changes, so does the modulation and therefore the data rate changes. Furthermore, nodes may come on- and off-line as interference changes the channel for higher frequency bands as it's expected in 6G.}
We propose to perform this activity offline. Detailed analysis is performed to unravel the security and performance strengths and weakness of the layers. Analysis is performed whenever there is a change in the hardware, operating system, libraries or the application layer. ASSESS builds a library of layers and will keep updating its knowledge whenever a new security exploit is reported.

MONITOR is a critical component in the architecture. In the preparatory phase, MONITOR is responsible for (i) recording benign resource usage ranges, (ii) tracking function to hardware mapping, and (iii) monitor the network to detect disruptive events within a short time. Discovery of the above information is vital to adapt the critical functionality as quickly as possible.

During the preparatory phase, ADAPT correlates the input(s) and output(s) of every critical function. It then discovers the relationship between them and acquires the necessary intelligence about the critical function to imitate it when required.

Adaptation phase kick starts a series of actions once a disruptive event is detected towards restoring critical functionality. When disruption happens, MONITOR first detects the disruption of critical functionality. It then triggers the COMPUTE component. At this stage, compute acquires the data discovered by MONITOR and ASSESS as presented in Fig.~\ref{fig:disrupt}. This is used to compute the new function to hardware mapping. This is fed as an input to the ADAPT component. It uses function's input to output correlation \raj{what is function intelligence?} to adapt it to the new full-stack.

% We will evaluate the integrated architecture in a simulated environment first and then on test beds utilizing resources from Chameleon, FABRIC and our partner application communities. \raj{I rewrote this sentence. Please check.} 
%To evaluate the integrated environment, we will perform detailed simulations and based on availability evaluate this on real-world deployments.

\begin{figure}
  \centering
  \includegraphics[trim=190 150 100 20,clip,width=\columnwidth]{figs/rings-at-disruption.png}
  \vspace{1mm}
  \caption{Disruption phase}
  \vspace{1mm}
  \label{fig:disrupt}
\end{figure}

==> sections/motivation.tex <==
\section{Motivation} \label{sec:motivation}

To illustrate the need for a dynamic architecture in which application roles are flexible, we present two network-based application use cases that could be deployed in future 6G networks.
Both systems described in this section are designed to protect human lives; therefore they must be resilient to disruptive events.

\subsection{Life-support system example}
Drawing analogy to "plain old" power grid, the producer and consumer in a power grid are not in the same location. Power transmission grid connects producers with consumers. Almost all components except transformers are passive. Transformer failures are prevented by performing preventive maintenance. Despite such a level of reliability, hospitals are expected to have backup power equipment to cover any power outage situation. 

%How far can we keep the situation under control ?
In the event of a disaster, unmanned control to the field becomes more critical. With  smart critical system, when the system collapses it negatively impacts human lives adversely much more than the impact of the actual disaster. 

To illustrate this let us go back to the hospital environment. This environment is designed to handle many disruptive scenarios but the life-support system may not survive a disaster situation such as an earthquake. Even when the patient survives the disaster, if the life-support system is dysfunctional, then it impacts the patient more than the disaster. These are the cases that we consider. This system is expected to hold the line until a rescue operation is launched.

%Will having more backups solve the problem ?
In the hospital example, having more backups will reduce the distance and hence the failure probability. It is worth noting that IoT smart critical system is moving away from proximal solutions. A sensor and its actuator counter-part cannot be co-located for a variety of reasons. For instance, fire in one part of a building must open an emergency door in a different location to provide an escape route. Apart from this, for techno-economic reasons, cloud computing and remote connectivity makes the distributed system affordable to the masses covering a wide variety of day-to-day use cases. A smart critical system that is both affordable and reliable is required.

Being adaptive is a time-tested solution to our survival on this planet. Being a similar survival (life or death) situation, we envision being adaptive as the solution to survival of this 6G network. Adaptive, not just to handful failure scenarios and resisting a few well-known security attacks but being adaptive even in an unexpected situation. Instead of studying resistance to single, and double failures, we should be looking at a $N-\epsilon$ ($\epsilon$ is as small as possible) failure resistance is the ultra-high reliability we should aim for. As for security attacks, resisting a new security attack is the key.

\subsection{Sea Level Measurement} \label{sec:sea-level}
Climate change has made flooding events in coastal areas more frequent and damaging. Deploying water level sensor through flood prone areas will help emergency response teams plan and respond during these events by getting access to real-time sea level measurements. Typically, an IoT-based sea level measurement system is composed of wireless water level sensors that send data to an IoT gateway. The IoT gateway aggregates and forwards data to an analysis (and storage) service in the Edge or Cloud, usually through a wireless link. 

Because most of the critical functions for this architecture reside on the wireless part of the network, the system can suffer from network intermittence during heavy rain events that cause flooding. Some systems can rely on local storage to store measurements and release them when the network connectivity is available. They can also rely on historical data to predict sea levels on a short time span. However, these solutions sacrifice the real-time nature of the system. We require new resiliency architectures that maintain the real-time nature of critical functions during disruptions.

\subsection{Tactical Defense} \label{sec:tac-defense}
Tactical defense networks are deployed in the battlefield to help troops communicate and coordinate. This environment opens a plethora of challenges. Where other networks are built to endure less stress and strain, tactical networks must operate in highly malicious environment and with multiple failures. The ability to defend against the enemy even when most communication and computing resources are lost becomes a base expectation of this network. In this highly dynamic scenario, resiliency is the key to protect critical functions. Depending on the isolation level, this network must function using cloud based resources to edge/fog resources all the way up to maintaining critical functionality with scarcely available resources. Due to multiple failures, a small set of resources can become isolated and these "resources" in traditional sense may not be sufficient to fully maintain the critical functionality. The resource scarcity must be overcome by mobilizing any available hardware and resources. This is a big challenge. It requires a dynamic architecture beyond the current state-of-the-art to realize critical functions from available resources.


